FPT Algorithms for Diverse Collections of Hitting Sets

In this work, we study the $d$-Hitting Set and Feedback Vertex Set problems through the paradigm of finding diverse collections of $r$ solutions of size at most $k$ each, which has recently been introduced to the field of parameterized complexity [Baste et al., 2019]. This paradigm is aimed at addressing the loss of important side information which typically occurs during the abstraction process which models real-world problems as computational problems. We use two measures for the diversity of such a collection: the sum of all pairwise Hamming distances, and the minimum pairwise Hamming distance. We show that both problems are FPT in $k + r$ for both diversity measures. A key ingredient in our algorithms is a (problem independent) network flow formulation that, given a set of `base' solutions, computes a maximally diverse collection of solutions. We believe that this could be of independent interest.

==> abstract.tex <==
\begin{abstract}
	In this work, we study the \dHS and \FVS problems through the paradigm of
  finding diverse collections of $r$ solutions of size at most $k$ each, which
  has recently been introduced to the field of parameterized complexity [Baste
  et al., 2019]. This paradigm is aimed at addressing the loss of important
  \emph{side information} which typically occurs during the abstraction process
  which models real-world problems as computational problems. We use two
  measures for the diversity of such a collection: the sum of all pairwise
  Hamming distances, and the minimum pairwise Hamming distance. We show that
  both problems are FPT in $k + r$ for both diversity measures. A key ingredient
  in our algorithms is a (problem independent) network flow formulation that,
  given a set of `base' solutions, computes a maximally diverse collection of
  solutions. We believe that this could be of independent interest.
\end{abstract}


==> notations.tex <==

\subsection{Overview of Notations and Terminology}

(not for inclusion in the final version)
This is supposed to help us to see any notation clashes.

\begin{itemize}[noitemsep]
\item concept of \emph{solution}
\item $r$ ``diverse'' solutions
  
\item of size $\le k$.
\item $n$ size of the ground set.
\item $U$ = ground set = universe. ($=V(G)$)
\item $n$ number of vertices
\item $\mathcal{S}$ all minimal solutions. (vertex covers, feedback
  vertex sets). Or a superset.
\item $F,G$, $F_1,\ldots,F_r$, $F_i$ ... solutions (clash with graph $G$!)
\item $S,T$, $S_1,\ldots,S_r$, $S_i$ ... solutions?

  
\item $d_H(F,G)$ Hamming distance
  $\Hammingdistance(F,G)$. or maybe
  $\Delta(F,G)$
\item a name for the SUM OBJECTIVE: 
$  \sumdiversity$
\item a name for the MIN OBJECTIVE: 
$  \mindiversity$
  
\item graph $G$.
\item graph $G=(V,E)$?
  
\item vertices $j=1,\ldots,n$.
\item $L_1,...L_b$; $L_q$ sets in the second definition of ``class''.
  and the corresponding nodes of the network.
  (Is there a more specific name for ``class''??)

\end{itemize}


(If you use some conflicting notations, just add them here anyway.
Or propose a better solution write it here first before changing
everything)

\tableofcontents


